Efficient Authentication of Outsourced String Similarity Search

Cloud computing enables the outsourcing of big data analytics, where a third party server is responsible for data storage and processing. In this paper, we consider the outsourcing model that provides string similarity search as the service. In particular, given a similarity search query, the service provider returns all strings from the outsourced dataset that are similar to the query string. A major security concern of the outsourcing paradigm is to authenticate whether the service provider returns sound and complete search results. In this paper, we design AutoS3, an authentication mechanism of outsourced string similarity search. The key idea of AutoS3 is that the server returns a verification object VO to prove the result correctness. First, we design an authenticated string indexing structure named MBtree for VO construction. Second, we design two lightweight authentication methods named VS2 and EVS2 that can catch the service provider various cheating behaviors with cheap verification cost. Moreover, we generalize our solution for top k string similarity search. We perform an extensive set of experiment results on real world datasets to demonstrate the efficiency of our approach.

==> framework.tex <==
–\section{The Framework}

Consider a data owner (client) who has a string dataset $D$ that contain $n$ string values $\{s_1, \dots, s_n\}$. He outsources $D$ and a similarity threshold $\theta$ to the third-party service provider (server), asking  the server to find all similar strings in $D$ with respect to their edit distance and $\theta$. Besides the similar string pairs, the client requires {\em a  proof of result correctness}. 

To construct the correctness proof, the client constructs the $MB^{ed}$ tree $T$ on $D$, and signs the digest of the root node of $T$. The client maintains the signature of the root node locally, and sends $D$ and $T$  to the server.  The server finds all similar pairs $P$ in $D$, constructs $VO$ of $P$, and sends $P$ and $VO$ back to the client for correctness verification.  To be more specific, 
for each string $s\in D$, its $VO$ $VO_s$ consists of its resulting similar strings $R(s)$, its dissimilar strings  $DS(s) = D - \{s\} - R(s)$, and the signature of a set of nodes in $T$ (more details of these nodes will be discussed in Section \ref{}). Upon receiving the $VO_s$, the client first checks the correctness by reconstructing the digest of
root of the $MB^{ed}$ tree from the $VO_s$ and then verifying it
against the root signature that is locally maintained. If the verification is successful, the client next finds
the result directly from the
data points extracted from the $VO_s$, and verifies the edit distance between the resulting strings and $s$. 
If the server omits some strings in the above $VO_s$,
then the client cannot reconstruct the correct root signature
in the above verification process. 

\nop{
Given a dataset $D$ containing $n$ string values $\{s_1, \dots, s_n\}$, and a edit distance threshold value $\theta$, the client firstly builds a Merkle B$^{ed}$ tree $T$ on the set of string values. Besides, the client also embeds the string values into a set of Euclidean points $P=\{p_1, \dots, p_n\}$. The framework is displayed in Figure \ref{fig:framework}.
\nop{
From the embeded points, the client generates a new threshold value $\theta'$ in Euclidean space such that 
\begin{equation}
Prob(DST(s_i, s_j)>\theta |DST(p_i, p_j)>\theta ') \geq \alpha,
\label{eq:prime}
\end{equation}
where $\alpha$ is a value between 0 and 1 specified by the client. After that, the client sends $D$, $T$ and $P$ to the server, along with $\theta$ and $\theta'$. 
}

\begin{figure}
\begin{center}
	\includegraphics[width=0.4\textwidth]{../figs/framework.eps}
	\caption{The verification framework}
	\label{fig:framework}
\end{center}
\end{figure}

For every string value $s \in D$, the server finds its similar string values. 
}

==> mb2.tex <==
The leaf node entry in the $MB^{ed}$-tree is of the form $(s, p, h)$, where $s$ is the string value, $p$ is the pointer to the disk block that stores $s$, and $h=Hash(s)$. The maximum number of entries in a leaf node is $f_1=\frac{P}{|p|+|s|+|h|}$. The internal node's entry is $(s^b, p, h, s^e)$, where $s^b$ and $s^e$ are the first and last string existing in the subtree rooted at the child node following the $B^{ed}$-tree's string ordering scheme, and $p$ points to the corresponding child node. An internal node can have at most $f_2=\frac{P}{|p|+|h|+2|s|}$ children nodes. The hash value in an entry is $h=Hash(s^b||h_1||dots||h_{f_2}||s^e)$. Let $N_R$ denote the root node. The client takes the hash value from the concatenation of $s^b$, $s^e$ and the hash value of every entry in the root node and takes the it as the $MB^{ed}$-tree's signature. An example of the $MB^{ed}$-tree structure is presented in Figure \ref{fig:mbtree}.

\begin{equation}
f_2=\frac{P}{2|s|+|h|+|p|},
\label{eq:f2}
\end{equation}
where $|h|$ is the length of a hash value, and $|p|$ is the point's size.

\begin{figure}
\begin{center}
	\includegraphics[width=0.4\textwidth]{../figs/mb2.eps}
	\caption{The structure of MBTree}
	\label{fig:mbtree}
\end{center}
\end{figure}

==> mbtree1.tex <==
The leaf node is identical to that of the $B^{ed}$ tree, where each entry contains a string value. The maximum number of strings residing in a leaf node is 
\begin{equation}
f_1=\frac{P}{|s|},
\label{eq:f1}
\end{equation}
where $P$ is the page size, and $|s|$ is the maximum size of a string value.  

The internal node's entry is of the form $(s^b, p, h, s^e)$, where $s^b$ and $s^e$ are the first and last string existing in the subtree rooted at the child node following the $B^{ed}$-tree's string ordering scheme, and $p$ points to the corresponding child node. We say that all leaf nodes' level is 0. A leaf node can have at most $f_2$ (Equation \ref{eq:f2}) children nodes. If the internal node's level is 1, $h=Hash(s_1||s_2||\dots||s_{f_1})$, where $s_1, \dots, s_{f_1}$ are the strings in the child leaf node. Otherwise, $h=Hash((s^b_1, h_1, s^e_1)||\dots||(s^b_{f_2}, h_{f_2}, s^e_{f_2}))$, which is generated from all of its children internal nodes. The client takes the hash value of the root node as the signature of the $MB^{ed}$-tree. Figure \ref{fig:mbtree} gives an example to illustrate the structure of a $MB^{ed}$-tree.

\begin{equation}
f_2=\frac{P}{2|s|+|h|+|p|},
\label{eq:f2}
\end{equation}
where $|h|$ is the length of a hash value, and $|p|$ is the point's size.

\begin{figure}
\begin{center}
	\includegraphics[width=0.4\textwidth]{../figs/mb1.eps}
	\caption{The structure of MBTree}
	\label{fig:mbtree}
\end{center}
\end{figure}

==> mbtree2.tex <==
The leaf node entry in the $MB^{ed}$-tree is of the form $(s, p, h)$, where $s$ is the string value, $p$ is the pointer to the disk block that stores $s$, and $h=Hash(s)$. The maximum number of entries in a leaf node is $f_1=\frac{P}{|p|+|s|+|h|}$. The internal node's entry is $(s^b, p, h, s^e)$, where $s^b$ and $s^e$ are the first and last string existing in the subtree rooted at the child node following the $B^{ed}$-tree's string ordering scheme, and $p$ points to the corresponding child node. An internal node can have at most $f_2=\frac{P}{|p|+|h|+2|s|}$ children nodes. The hash value in an entry is $h=Hash(s^b||h_1||dots||h_{f_2}||s^e)$. Let $N_R$ denote the root node. The client takes the hash value from the concatenation of $s^b$, $s^e$ and the hash value of every entry in the root node and takes the it as the $MB^{ed}$-tree's signature. An example of the $MB^{ed}$-tree structure is presented in Figure \ref{fig:mbtree}.

\begin{equation}
f_2=\frac{P}{2|s|+|h|+|p|},
\label{eq:f2}
\end{equation}
where $|h|$ is the length of a hash value, and $|p|$ is the point's size.

\begin{figure}
\begin{center}
	\includegraphics[width=0.4\textwidth]{../figs/mb2.eps}
	\caption{The structure of MBTree}
	\label{fig:mbtree}
\end{center}
\end{figure}
